Struct-MDC: Mesh-Refined Unsupervised Depth Completion Leveraging Structural Regularities from Visual SLAM

Feature-based visual simultaneous localization and mapping (SLAM) methods only estimate the depth of extracted features, generating a sparse depth map. To solve this sparsity problem, depth completion tasks that estimate a dense depth from a sparse depth have gained significant importance in robotic applications like exploration. Existing methodologies that use sparse depth from visual SLAM mainly employ point features. However, point features have limitations in preserving structural regularities owing to texture-less environments and sparsity problems. To deal with these issues, we perform depth completion with visual SLAM using line features, which can better contain structural regularities than point features. The proposed methodology creates a convex hull region by performing constrained Delaunay triangulation with depth interpolation using line features. However, the generated depth includes low-frequency information and is discontinuous at the convex hull boundary. Therefore, we propose a mesh depth refinement (MDR) module to address this problem. The MDR module effectively transfers the high-frequency details of an input image to the interpolated depth and plays a vital role in bridging the conventional and deep learning-based approaches. The Struct-MDC outperforms other state-of-the-art algorithms on public and our custom datasets, and even outperforms supervised methodologies for some metrics. In addition, the effectiveness of the proposed MDR module is verified by a rigorous ablation study.

==> 6.acknowledgement.tex <==
\section*{ACKNOWLEDGMENT}

The preferred spelling of the word ``acknowledgment'' in America is without an ``e'' after the ``g''. Avoid the stilted expression, ``One of us (R. B. G.) thanks . . .''  Instead, try ``R. B. G. thanks''. Put sponsor acknowledgments in the unnumbered footnote on the first page.

==> results.tex <==


\begin{table}[!th]
\centering
\renewcommand{\arraystretch}{1.5} % height
\renewcommand{\tabcolsep}{0.9mm}  % width 
\caption{Quantitative comparison results with state-of-the-arts on VOID. 
(
    \textit{pre}: results using their pretrained weight. 
    \textit{re}: results using retrained weight.
    %\textbf{U}: unsupervised method, \textbf{S}: supervised method
    $\downarrow$: lower the better and $\uparrow$: higher the better.
)}

\begin{tabular}{lccccccc}
\hline
\multicolumn{2}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Error {[}mm{]} $\downarrow$} &  & \multicolumn{3}{c}{Accuracy {[}\%{]} $\uparrow$}    \\ \cline{3-4} \cline{6-8} 
\multicolumn{2}{c}{}                        & MAE                    & RMSE                   &  & $\delta_1$      & $\delta_2$      & $\delta_3$      \\ \hline
\multirow{2}{*}{VOICED}             & (pre) & 167.608                & 316.017                &  & 57.499          & 74.014          & 96.974          \\
                                    & (re)  & 162.272                & 284.562                &  & 36.166          & \textbf{75.072} & 98.430          \\
\multirow{2}{*}{ScaffNet-FusionNet} & (pre) & 167.600                & 346.533                &  & 55.455          & 72.721          & 97.866          \\
                                    & (re)  & 166.143                & 337.522                &  & 58.841          & 73.894          & 96.346          \\
KBNet (baseline)                    & (re)  & 143.801                & 262.643                &  & 52.286          & 69.494          & 98.724          \\
Ours                                &       & \textbf{111.332}       & \textbf{216.497}       &  & \textbf{62.074} & 74.544          & \textbf{99.003} \\ \hline
\end{tabular}

\label{table:exp_void}
\vspace{-0.2cm}
\end{table}


\begin{figure}[th!]
        \begin{subfigure}[b]{0.166\columnwidth}
                \includegraphics[width=\textwidth]{figure/void_2d_rgbd_point.pdf}
                \caption{}
                \label{fig:void_point}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \includegraphics[width=\textwidth]{figure/void_2d_rgbd_line.pdf}
                \caption{}
                \label{fig:void_line}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/void_2d_voiced.pdf}
                \caption{\cite{void}}
                \label{fig:void_voiced}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/void_2d_kbnet.pdf}
                \caption{\cite{baseline}}
                \label{fig:void_baseline}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/void_2d_my.pdf}
                \caption{Ours}
                \label{fig:void_ours}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/void_2d_gt.pdf}
                \caption{GT}
                \label{fig:void_gt}
        \end{subfigure}
        \caption{
        Qualitative comparison results on VOID: 
        (a) point features (b) point and line features from VI-SLAM,
        completed depth from (c)-(e),  and
        ground-truth depth}\label{fig:void_result}
\vspace{-0.5cm}
\end{figure}





% \vspace{-0.5cm}
\section{RESULTS WITH ANALYSIS}\label{sec:result}


\begin{figure*}[th!]
    % \vspace{-0.25cm}
    \centering
    \includegraphics[width=18cm, height=5.5cm]{figure/3d_visualize.pdf}
    \caption{3D visualization of estimated depth on VOID (left three columns) and NYUv2 (right three columns): Detected features (top row), estimated depth from our baseline (middle row), and proposed method (bottom row). Proposed method clearly aligns object boundary with reduced jittering.} 
    \label{fig:3d_visualize}
    \vspace{-0.4cm}
\end{figure*} 


realistic situation을 가정하여, 우리는 실험을 진행한 모든 데이터셋에 대해 VOID \cite{void}의 가장 낮은 density인 $0.05\%$ 에 해당하는 총 150 개의 feature를 추출하여 사용했다.
우리가 제안한 방법은 line feature라는 새로운 measurement를 사용하므로 공정한 비교를 위해 line feature를 추출하는 경우 line feature와 point feature 개수의 총합이 150이 되도록 제한했다. 
정확한 비교를 위해, 실험에 사용된 모든 비교군은 각 dataset에서 retrained되었다.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3-1) 실험: VOID dataset 
\subsection{Comparison on VOID Dataset}

% 질적 비교 분석
man-made environment에서는 Fig. \ref{fig:void_line}와 같이 object boundary에 많은 line feature가 관찰된다. 따라서 기존의 방법론에 비해, 제안된 방법론에서 object가 더 명확히 추정되는 것을 Fig. \ref{fig:void_result}에서 확인할 수 있다.  
% DT vs. CDT의 위력
line feature를 도입함에 따른 장점은 CDT로부터 발생하는 효과와 line feature 자체로부터 파생되는 효과로 구분될 수 있다. 
전자의 경우, 오직 point feature로부터의 triangulation에 의존하는 \cite{void}는 서로 다른 object에 속한 feature간에 triangle이 형성되는 경우가 많다. 따라서 Fig. \ref{fig:void_voiced}와 같이 triangulation의 흔적이 존재하는 모호한 depth가 추정된다. 하지만 제안된 방법론은 object의 boundary를 포함한 triangle을 형성하므로 object간의 구분이 명확하다. 
% 더 정확한 object boundary를 포착할수록, 해당 object 내부의 depth도 더 정확하게 채울 수 있다. 
후자의 경우, 다른 방법론이 놓치는 경계선들이 우리의 방법론에서는 line feature로써 포함되어 있으므로 최종 결과물에서도 이 경계선들이 좀 더 명확하게 나타난다. 주목할 만한 점은, 원형 탁자와 같은 곡선 경계 또한 우리의 piece-wise linear가정에 따라 명확하게 추정할 수 있다는 것이다. 
% baseline과의 비교
우리의 baseline \cite{baseline}은 여전히 몇몇 scene에서 stain이 나타난다. 그들은 point feature의 낮은 density를 채우기 위해 pooling layer에 크게 의존하므로 최종 결과물에도 copy and paste의 흔적이 남아있는 것으로 분석된다. 이에 비해, 제안된 방법론은 empty space를 채우기 위해 interpolation 및 MDR를 순차적으로 사용해 각 모듈의 역할을 분담함으로써 이러한 stain을 없애고 전반적인 성능을 끌어올렸다. 
% 양적 비교 분석
이러한 성능 향상이 Table. \ref{table:exp_void}에 수치적으로 나타난다. 제안된 방법론에서는 state-of-the-art인 \cite{baseline}에 비해 MAE와 RMSE가 각각 $22.58\%$, $17.57\%$ 만큼 향상되었으며 accuracy도 state-of-the-art의 성능을 달성했다.
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3-2) 실험: NYU-Depth-v2 
\begin{table}[!th]
\centering
\renewcommand{\arraystretch}{1.5} % height
\renewcommand{\tabcolsep}{0.9mm}  % width 
\caption{Quantitative comparison results with state-of-the-arts on NYUv2.
(
    \textit{pre}: results using their pretrained weight. 
    \textit{re}: results using retrained weight.
    \textbf{U}: unsupervised, \textbf{S}: supervised
    $\downarrow$: lower the better and $\uparrow$: higher the better.
)}

\begin{tabular}{lcccccccc}
\hline
\multicolumn{3}{c}{Method}                                       & \multicolumn{2}{c}{Error {[}mm{]} $\downarrow$} & \multicolumn{1}{l}{} & \multicolumn{3}{c}{Accuracy {[}\%{]} $\uparrow$}    \\ \cline{4-5} \cline{7-9} 
\multicolumn{3}{c}{}                                             & MAE                    & RMSE                   & \multicolumn{1}{l}{} & $\delta_1$      & $\delta_2$      & $\delta_3$      \\ \hline
\multirow{2}{*}{VOICED}             & \multirow{2}{*}{U} & (pre) & 244.416                & 407.979                &                      & 54.488          & 71.107          & 97.255          \\
                                    &                    & (re)  & 205.898                & 328.202                &                      & 56.965          & 74.747          & 99.401          \\
\multirow{2}{*}{ScaffNet-FusionNet} & \multirow{2}{*}{U} & (pre) & 223.111                & 353.720                &                      & 51.878          & 69.801          & 99.282          \\
                                    &                    & (re)  &                        &                        &                      &                 &                 &                 \\
KBNet (baseline)                    & U                  & (re)  & 179.817                & 297.872                &                      & 59.605          & 78.027          & 99.346          \\
Ours                                & U                  &       & \textbf{141.871}       & \textbf{245.548}       &                      & \textbf{67.991} & \textbf{81.999} & \textbf{99.698} \\ \hline
CSPN                                & S                  &       & \textbf{163.152}       & \textbf{245.864}       &                      & 59.092          & \textbf{84.656} & \textbf{99.861} \\
Ours                                & U                  &       & \textbf{141.871}       & \textbf{245.548}       &                      & \textbf{67.991} & 81.999          & 99.698          \\ \hline
\end{tabular}

\label{table:exp_nyu}
\vspace{-0.3cm}
\end{table}

\begin{figure}[th!]
        \begin{subfigure}[b]{0.166\columnwidth}
                \includegraphics[width=\textwidth]{figure/nyu_2d_rgbd_point.pdf}
                \caption{}
                \label{fig:nyu_point}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \includegraphics[width=\textwidth]{figure/nyu_2d_rgbd_line.pdf}
                \caption{}
                \label{fig:nyu_line}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/nyu_2d_voiced.pdf}
                \caption{\cite{void}}
                \label{fig:nyu_voiced}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/nyu_2d_kbnet.pdf}
                \caption{\cite{baseline}}
                \label{fig:nyu_baseline}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/nyu_2d_my.pdf}
                \caption{Ours}
                \label{fig:nyu_ours}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/nyu_2d_gt.pdf}
                \caption{GT}
                \label{fig:nyu_gt}
        \end{subfigure}
        \caption{
        Qualitative comparison results on NYUv2: 
        (a) point features (b) point and line features from VI-SLAM,
        completed depth from (c)-(e),  and
        ground-truth depth}\label{fig:nyu_result}
        \vspace{-0.5cm}
\end{figure}

\subsection{Comparison on NYUv2 Dataset}

질적인 비교 결과가 Fig. \ref{fig:nyu_result}에 나타난다. 이 실험에서도 \cite{void}에서는 triangulation의 흔적이 남아있으며 \cite{baseline}에서는 stain이 관측된다. 하지만 line feature를 사용하는 우리의 방법론은 ground-truth와 육안으로 보기에 근접한 depth를 추정한다. 특히 제안된 방법론은 Fig. \ref{fig:nyu_result}의 첫번째 row와 같이 texrueless하여 point feature가 추출되지 않는 영역이나 네번째 row와 같이 구조적인 object에서 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!th]
\centering
\renewcommand{\arraystretch}{1.5} % height
\renewcommand{\tabcolsep}{0.9mm}  % width 
\caption{\textcolor{red}{(임시)} Quantitative comparison results with state-of-the-arts on PLAD.
(
    \textit{pre}: results using their pretrained weight. 
    \textit{re}: results using retrained weight.
    \textbf{U}: unsupervised, \textbf{S}: supervised
    $\downarrow$: lower the better and $\uparrow$: higher the better.
)}

\begin{tabular}{lcccccccc}
\hline
\multicolumn{3}{c}{Method}                                       & \multicolumn{2}{c}{Error {[}mm{]} $\downarrow$} &  & \multicolumn{3}{c}{Accuracy {[}\%{]} $\uparrow$}    \\ \cline{4-5} \cline{7-9} 
\multicolumn{3}{c}{}                                             & MAE                    & RMSE                   &  & $\delta_1$      & $\delta_2$      & $\delta_3$      \\ \hline
\multirow{2}{*}{VOICED}             & \multirow{2}{*}{U} & (pre) & 244.416                & 407.979                &  & 54.488          & 71.107          & 97.255          \\
                                    &                    & (re)  & 205.898                & 328.202                &  & 56.965          & 74.747          & 99.401          \\
\multirow{2}{*}{ScaffNet-FusionNet} & \multirow{2}{*}{U} & (pre) &                        &                        &  &                 &                 &                 \\
                                    &                    & (re)  &                        &                        &  &                 &                 &                 \\
KBNet (baseline)                    & U                  & (re)  & 179.817                & 297.872                &  & 59.605          & 78.027          & 99.346          \\
Ours                                & U                  &       & \textbf{141.871}       & \textbf{245.548}       &  & \textbf{67.991} & \textbf{81.999} & \textbf{99.698} \\ \hline
CSPN                                & S                  &       & 163.152                & 245.864                &  & 59.092          & \textbf{84.656} & \textbf{99.861} \\
Ours                                & U                  &       & \textbf{141.871}       & \textbf{245.548}       &  & \textbf{67.991} & 81.999          & 99.698          \\ \hline
\end{tabular}

\label{table:exp_plad}
\vspace{-0.35cm}
\end{table}
\begin{figure}[th!]
        \begin{subfigure}[b]{0.166\columnwidth}
                \includegraphics[width=\textwidth]{figure/nyu_2d_rgbd_point.pdf}
                \caption{}
                \label{fig:plad_point}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \includegraphics[width=\textwidth]{figure/nyu_2d_rgbd_line.pdf}
                \caption{}
                \label{fig:plad_line}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/nyu_2d_voiced.pdf}
                \caption{\cite{void}}
                \label{fig:plad_voiced}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/nyu_2d_kbnet.pdf}
                \caption{\cite{baseline}}
                \label{fig:plad_baseline}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/nyu_2d_my.pdf}
                \caption{Ours}
                \label{fig:plad_ours}
        \end{subfigure}%
        \begin{subfigure}[b]{0.166\columnwidth}
                \centering
                \includegraphics[width=\textwidth]{figure/nyu_2d_gt.pdf}
                \caption{GT}
                \label{fig:plad_gt}
        \end{subfigure}
        \caption{ \textcolor{red}{(임시)} 
        Qualitative comparison results on PLAD: 
        (a) point features (b) point and line features from VI-SLAM,
        completed depth from (c)-(e),  and
        ground-truth depth}\label{fig:plad_result}
        \vspace{-0.5cm}
\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
상대적으로 더 큰 빛을 발휘한다. 
% 양적 비교 분석
이러한 성능 향상이 Table. \ref{table:exp_nyu}에 수치적으로 나타난다. 제안된 방법론에서는 state-of-the-art인 \cite{baseline}에 비해 MAE와 RMSE가 각각 $21.10\%$, $17.57\%$ 만큼 향상되었으며 accuracy도 state-of-the-art의 성능을 달성했다. 
주목할 만한 점은, 제안된 방법론은 unsupervised 방식임에도 불구하고, error metric과 accuracy metric of $\delta_1$에서 supervised 방식인 CSPN \cite{cspn}의 성능을 능가한다는 것이다.
% 3D 비교
명확한 비교를 위해, Fig. \ref{fig:3d_visualize}는 VOID와 NYUv2에서 baseline \cite{baseline}과 제안된 방법론이 추정한 3D depth를 보여준다. \cite{baseline}는 object의 boundary에서 jittering이 발생하여 부정확한 반면, 제안된 방법론에서는 이것이 상당히 감소하여 정확한 depth가 추정되었다. object의 boundary를 정확하게 포착함으로써 object 내부의 depth도 더 정확하게 추정되었다.










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3-3) 실험: Custom Dataset 


\subsection{Comparison on PLAD Dataset}

\textcolor{blue}{[실험 후 작성 예정] }
not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented.
% not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented.
% not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. not implemented. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 4) Ablation Study 
\subsection{Ablation Study}

%% 1.
\noindent
\textbf{Mesh depth Refinement module } 
제안된 MDR의 효과를 엄밀하게 입증하기 위해 두 종류의 데이터셋에서 ablation study가 수행됐다.
% 양적 비교
% One may think that ~
line feature를 사용할 경우 당연하게도 주어진 prior가 증가하여 모델의 성능이 더 좋아질 것이라고 생각할 수 있다. 이것은 Table \ref{table:ablation_1}에서 확인될 수 있듯이 사실이다. 하지만 단순히 line feature를 model의 input으로 사용하는 것은 line의 potential을 제대로 사용한다고 보기 어렵다.
실제로 단순히 point와 line feature를 baseline model에 사용한 경우 (P+L)와 비교했을 때, 제안된 방법론 (P+L+M+R)은 전체적인 성능을 dramatically 향상시켰다.
% 질적 비교
qualitative comparison을 위해, Fig. \ref{fig:error_plot}는 point와 line을 단순히 input으로 사용한 경우 (P+L), CDT mesh를 input으로 사용한 경우 (P+L+M), 그리고 제안된 MDR 모듈을 사용한 경우 (P+L+M+R)에 대한 error plot을 보여준다. 
% 공통적인 관찰 정보
% 예상되었던 바와 같이, 가까운 거리의 object에 비해 공통적으로 먼 거리의 object에서 depth estimation의 error가 큰 것을 관찰할 수 있다. 이는 실제로 먼 거리에 위치한 pixel일수록 disparity가 작아 photometric consistency loss $l_s$에서 사용된 reconstruction이 errneous해지기 때문이다.
% 각 방법론 비교
단순히 point와 line을 사용했을 때보다, CDT를 통한 mesh를 사용했을 때 전체적인 error가 작아졌으며, mesh refinement를 추가로 수행했을 경우 error가 더 작아졌다. 
% P의 한계
naive하게 line feature를 network의 추가 input으로 이용할 경우, 여전히 object의 boundary에서 blur hole이 존재한다. 
% 이러한 blur hole은 실제 ground-truth depth가 continous한 영역에서도 관측된다.
% Fig. \ref{fig:error_plot}에 visualize된 error $e$는 estimated depth $\hat{D}$와 ground-truth $D$간의 absolute difference로 정의되므로 
% 이는 estimated depth에도 blur hole이 존재한다는 것을 의미한다. 
이는 학습을 위해 사용된 local smoothness loss $l_l$에서 object boundary의 depth discontinuity를 accomodate하기 위한 penalty가 크게 작용하여 네트워크가 단순히 copy and paste만을 수행하는 local minima에 빠졌음을 암시한다. 우리의 baseline은 densify를 위해 pooling layer를 사용하므로 모델이 이러한 local minima에 빠질 가능성이 높다. 
% M의 장점
이와 대조적으로, interpolated mesh depth가 input으로 이용된 경우, object의 boundary가 잘 포착되면서도 이러한 blur hole이 제거되었다. 이는 line을 사용한 CDT를 통해 object boundary를 aware하면서도 interpolation을 통해 빈 depth가 채워졌기 때문이다. 
% R의 장점
mesh를 사용했을 때의 이러한 장점은 제안된 모듈 MDR를 사용할 경우 시너지를 발휘한다.






\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.5} % height
\renewcommand{\tabcolsep}{1.1mm}  % width 
\caption{Ablation study: Effectiveness of the proposed Mesh Depth Refinement module. (
    \textbf{P}: point feature, \textbf{L}: line feature, \textbf{M}: interpolated mesh, \textbf{R}: proposed refinement module.
    $\downarrow$: lower the better and $\uparrow$: higher the better.
)}

\begin{tabular}{clcccccc}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Error {[}mm{]} $\downarrow$} &  & \multicolumn{3}{c}{Accuracy {[}\%{]} $\uparrow$}    \\ \cline{3-4} \cline{6-8} 
                         & \multicolumn{1}{c}{}                        & MAE                    & RMSE                   &  & $\delta_1$      & $\delta_2$      & $\delta_3$      \\ \hline
\multirow{4}{*}{VOID}    & P (baseline)                                & 143.801                & 262.643                &  & 52.286          & 69.494          & 98.724          \\
                         & P + L                                       & 124.243                & 235.622                &  & 58.642          & 72.745          & 98.949          \\
                         & P + L + M                                   & 120.917                & 228.467                &  & 58.741          & 73.418          & 99.002          \\
                         & P + L + M + R                               & \textbf{111.332}       & \textbf{216.497}       &  & \textbf{62.074} & \textbf{74.544} & \textbf{99.003} \\ \hline
\multirow{4}{*}{NYUv2}   & P (baseline)                                & 179.817                & 297.872                &  & 59.605          & 78.027          & 99.346          \\
                         & P + L                                       & 163.618                & 270.276                &  & 62.230          & 79.185          & 99.500          \\
                         & P + L + M                                   & 145.980                & 250.174                &  & 67.175          & 81.571          & 99.706          \\
                         & P + L + M + R                               & \textbf{141.871}       & \textbf{245.548}       &  & \textbf{67.991} & \textbf{81.999} & \textbf{99.698} \\ \hline
\end{tabular}

\label{table:ablation_1}
\vspace{-0.3cm}
\end{table}

\begin{figure}[th!]
    % \vspace{-0.25cm}
    \centering
    \includegraphics[width=8.7cm, height=1.9cm]{figure/error_plot.pdf}
    \caption{Error plot of different input method with ground-truth depth. In the three error figures on the right, the brighter the color, the greater the error.} 
    \label{fig:error_plot}
    \vspace{-0.5cm}
\end{figure} 






% %% 2.
% \noindent
% \textbf{Parallel pooling and discontinuity-aware channel } 
% In this section, 제안된 MDR module의 component를 도입한 효과가 분석된다. 
% 하지만, MDR module은 8-channel의 intermediate tensor를 estimate한다. 따라서 우리는 qualitative comparison을 위해 MDR module의 마지막 layer가 산출한 feature map을 visualize하여 분석한다.

% \begin{table}[!ht]
% \centering
% \renewcommand{\arraystretch}{1.5} % height
% \renewcommand{\tabcolsep}{0.5mm}  % width 
% \caption{Ablation study: Effectiveness of the proposed Mesh Depth Refinement module components. (
%     $\downarrow$: lower the better and $\uparrow$: higher the better.
% )}

% \begin{tabular}{clccccc}
% \hline
% \multirow{2}{*}{Dataset}                  & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Error {[}mm{]} $\downarrow$} &  & \multicolumn{2}{c}{Accuracy {[}\%{]} $\uparrow$} \\ \cline{3-4} \cline{6-7} 
%                                           & \multicolumn{1}{c}{}                        & MAE                    & RMSE                   &  & $E(\hat{D}, 1.05)$      & $E(\hat{D}, 1.10)$     \\ \hline
% \multicolumn{1}{l}{\multirow{4}{*}{VOID}} & MDR                                         & 115.752                & 224.816                &  & 61.747                  & 74.082                 \\
% \multicolumn{1}{l}{}                      & MDR (+ m || M)                              & 114.435                & 221.490                &  & 61.230                  & 73.631                 \\
% \multicolumn{1}{l}{}                      & MDR (+ mask)                                & 116.049                & 223.324                &  & 61.097                  & 73.362                 \\
% \multicolumn{1}{l}{}                      & MDR (+ m || M \& mask)                      & \textbf{113.834}       & \textbf{220.396}       &  & \textbf{62.142}         & \textbf{74.389}        \\ \hline
% \multirow{4}{*}{NYUv2}                    & MDR                                         & 143.927                & 245.217                &  & 67.096                  & 81.658                 \\
%                                           & MDR (+ m || M)                              & 142.435                & 245.103                &  & 67.587                  & 81.924                 \\
%                                           & MDR (+ mask)                                & 143.143                & 245.461                &  & 67.633                  & 81.967                 \\
%                                           & MDR (+ m || M \& mask)                      & \textbf{142.231}       & \textbf{244.841}       &  & \textbf{67.758}         & \textbf{82.128}        \\ \hline
% \end{tabular}
% \label{table:ablation_2}
% \end{table}





